Privacy Vulnerability of Split Computing to Data-Free Model Inversion Attacks

Mobile edge devices see increased demands in deep neural networks (DNNs) inference while suffering from stringent constraints in computing resources. Split computing (SC) emerges as a popular approach to the issue by executing only initial layers on devices and offloading the remaining to the cloud. Prior works usually assume that SC offers privacy benefits as only intermediate features, instead of private data, are shared from devices to the cloud. In this work, we debunk this SC-induced privacy protection by (i) presenting a novel data-free model inversion method and (ii) demonstrating sample inversion where private data from devices can still be leaked with high fidelity from the shared feature even after tens of neural network layers. We propose Divide-and-Conquer Inversion (DCI) which partitions the given deep network into multiple shallow blocks and inverts each block with an inversion method. Additionally, cycle-consistency technique is introduced by re-directing the inverted results back to the model under attack in order to better supervise the training of the inversion modules. In contrast to prior art based on generative priors and computation-intensive optimization in deriving inverted samples, DCI removes the need for real device data and generative priors, and completes inversion with a single quick forward pass over inversion modules. For the first time, we scale data-free and sample-specific inversion to deep architectures and large datasets for both discriminative and generative networks. We perform model inversion attack to ResNet and RepVGG models on ImageNet and SNGAN on CelebA and recover the original input from intermediate features more than 40 layers deep into the network.

==> figs/abla_dci/dci_fig.tex <==
\begin{figure}[!t]
\centering
% \vspace{-8mm}
%%% please modify here

\begingroup
% \renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{c}
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figs/real_inv/inv/merged_inv.png}
% \\
\includegraphics[width=0.7\linewidth]{figs/abla_dci/dci_real.pdf} \\
\end{tabular}
%
\endgroup
% \vspace{1mm}

\small{\ \ Real images $\mathbf{x}$ from the ImageNet validation set.} \\


\begingroup
% \renewcommand*{\arraystretch}{0.3}
\begin{tabular}{c}
\includegraphics[width=0.7\linewidth]{figs/abla_dci/dci_yes.pdf} \\
%
\end{tabular}
\endgroup

\small{Inverted images by inversion model trained w/ DCI.\ \ \ (LPIPS $\downarrow$\ =\ 0.443)} \\


\begingroup
% \renewcommand*{\arraystretch}{0.3}
\begin{tabular}{c}
\includegraphics[width=0.7\linewidth]{figs/abla_dci/dci_no.pdf} \\
%
\end{tabular}
\endgroup

\small{Inverted images by inversion model trained w/o DCI. (LPIPS $\downarrow$\ =\ 0.497)} \\
\vspace{2mm}
\caption{Comparison of inversion attack with (and without) Divide-and-Conquer Inversion (DCI).
}
\vspace{-4mm}
\label{fig:abla_dci}
\end{figure}


==> figs/moco_inv/moco_inv.tex <==
\begin{figure}[H]
\centering
% \vspace{-8mm}
%%% please modify here

\begingroup
% \renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{c}
% \includegraphics[width=0.45\linewidth,clip,trim=5px 0 0 4px]{figs/real_inv/inv/merged_inv.png}
% \\
\includegraphics[width=0.95\linewidth]{figs/moco_inv/inv-moco-0.png} \\
\end{tabular}
%
\endgroup
% \vspace{1mm}

\small{\ \ Real images $\mathbf{x}$ from the ImageNet validation set.} \\


\begingroup
% \renewcommand*{\arraystretch}{0.3}
\begin{tabular}{c}
\includegraphics[width=0.95\linewidth]{figs/moco_inv/inv_sup_resnet50.png} \\
%
\end{tabular}
\endgroup

\small{Inverted images from ResNet-50's (supervised~\cite{He2015}) features after $42$ conv. layers.
% \scalebox{0.8}{$\mathcal{F}_{1:42}^{-1}(\mathcal{F}_{1:42}(\mathbf{x})\big)$}
} \\


\begingroup
% \renewcommand*{\arraystretch}{0.3}
\begin{tabular}{c}
\includegraphics[width=0.95\linewidth]{figs/moco_inv/inv-moco-1.png} \\
%
\end{tabular}
\endgroup

\small{Inverted images from ResNet-50's \\(MoCoV2~\citep{chen2020mocov2}) features after $42$ conv. layers.
% \scalebox{0.8}{$\mathcal{F}_{1:42}^{-1}(\mathcal{F}_{1:42}(\mathbf{x})\big)$}
} \\



\caption{Inversion attacks to ResNet-50 pre-trained by supervised and self-supervised learning without real data.}
\vspace{-2mm}
\label{fig:moco_main}
\end{figure}


==> figs/relate_comp/relate_comp.tex <==
\begin{wrapfigure}{r}{0.3\textwidth}
\vspace{-3mm}
\begin{minipage}{0.3\textwidth}
% \begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/relate_comp/bmvc-gmi.pdf}
    \caption{Comparison between our method and generative inversion methods. 
    Although inverted images from generative inversions are semantically close to the original ones, sample-level faithfulness between the inverted and the original images cannot be guaranteed.
    }
    \label{fig:relate_comp}
    \vspace{-3mm}
% \end{figure}
\end{minipage}
\end{wrapfigure}
